Checking Chase Termination over Ontologies of Existential Rules with Equality

The chase is a sound and complete algorithm for conjunctive query answering over ontologies of existential rules with equality. To enable its effective use, we can apply acyclicity notions; that is, sufficient conditions that guarantee chase termination. Unfortunately, most of these notions have only been defined for existential rule sets without equality. A proposed solution to circumvent this issue is to treat equality as an ordinary predicate with an explicit axiomatisation. We empirically show that this solution is not efficient in practice and propose an alternative approach. More precisely, we show that, if the chase terminates for any equality axiomatisation of an ontology, then it terminates for the original ontology (which may contain equality). Therefore, one can apply existing acyclicity notions to check chase termination over an axiomatisation of an ontology and then use the original ontology for reasoning. We show that, in practice, doing so results in a more efficient reasoning procedure. Furthermore, we present equality model-faithful acyclicity, a general acyclicity notion that can be directly applied to ontologies with equality.

==> sections/cemetry.tex <==


\begin{theorem}
Deciding BCQ entailment for ontologies \Tuple{\RuleSet, \FactSet} with \RuleSet an EMFA rule set is \DoubleExpTime-complete even if the arity of predicates is bounded.
\end{theorem}
\begin{proof}[Sketch]
(Base Case)
We have that $\AtomSet_0 \Rewriting_\star \subseteq \MFA{\RuleSet}$ since $\AtomSet_0 = \FactSet$ by Definition~\ref{definition:chase}, and $\FactSet_\star \subseteq \MFA{\RuleSet}$ by Definition~\ref{definition:emfa}.

(Induction Step)
Let $i \geq 1$.
By induction hypothesis, we have that

For all $i \geq 0$, let $\Rewriting_i$ be the rewriting defined as follows:
\begin{itemize}
	\item $\Rewriting_0$ is the empty function.
	\item For all $i \geq 1$, we consider two different cases:
	If $\AtomSet_i = \AtomSet_{i-1}[t / u]$ for some $t, u \in \GroundTerms$; then $\Rewriting_i = \Rewriting_{i-1} \circ [u / t]$ if $\Depth{t} < \Depth{u}$, and $\Rewriting_i = \Rewriting_{i-1} \circ [t / u]$ otherwise.
	Otherwise (i.e., if $\AtomSet_{i-1} \subseteq \AtomSet_i$), let $\Rewriting_i = \Rewriting_{i-1}$.
\end{itemize}
Let $\AtomSet_1', \AtomSet_2', \ldots$ be the sequence with $\AtomSet_i' = \AtomSet_i \Rewriting_i$ for all $i \geq 0$.
We verify that the chase sequence $\AtomSet_1, \AtomSet_2, \ldots$ is finite by showing that $\AtomSet_1', \AtomSet_2', \ldots$ is finite.

Let $\Rewriting_\star$ be the rewriting that maps every $t \in \GroundTerms$ to the term that results from replacing every syntactic occurrence of a constant in $t$ with $\star$.
We can show via induction that, for all $i \geq 0$, $\AtomSet_i'\Rewriting_\star \subseteq \MFA{\RuleSet}$.
Since \RuleSet is MFA, the atom set \MFA{\RuleSet} is finite and hence, an atom set in $\AtomSet_1', \AtomSet_2', \ldots$ may contain at most

the chase sequence $\AtomSet_1, \AtomSet_2, \ldots$ does terminate.

(Membership)
Membership is shown as for Theorem~\ref{}, since we obtain the same upper bound for the number of ground skolem terms that are not cyclic.

(Hardness)
Hardness is established by modifying the construction of a \DoubleExpTime Turing machine given for deterministic, weakly acyclic rules by Cal\`{i} et al. \shortcite{qa-non-guarded-rules}.
The construction yields a grid of doubly exponential size, using predicates of arity at mot $3$.
The remaining Turing machine simulation follows standard constructions (cf. \cite{complexity-logic-programming}), using elements of this grid to refer to specific time points and tape cells when encoding a run of the Turing machine.
\end{proof}

